Lambada: Interactive Data Analytics on Cold Data using Serverless Cloud Infrastructure

The promise of ultimate elasticity and operational simplicity of serverless computing has recently lead to an explosion of research in this area. In the context of data analytics, the concept sounds appealing, but due to the limitations of current offerings, there is no consensus yet on whether or not this approach is technically and economically viable. In this paper, we identify interactive data analytics on cold data as a use case where serverless computing excels. We design and implement Lambada, a system following a purely serverless architecture, in order to illustrate when and how serverless computing should be employed for data analytics. We propose several system components that overcome the previously known limitations inherent in the serverless paradigm as well as additional ones we identify in this work. We can show that, thanks to careful design, a serverless query processing system can be at the same time one order of magnitude faster and two orders of magnitude cheaper compared to commercial Query-as-a-Service systems, the only alternative with similar operational simplicity.

==> cvm.tex <==
\section{The Collection Virtual Machine (CVM)}
\label{sec:ir}

Several different types of data processing on the data-science level such as
relational algebra, graph analysis, linear algebra, and machine learning work on
relations of records, set of vertices and edges, vectors and matrices of
numbers, and bags of samples, respectively. All of these are some sort of
``collection'' of ``tuples'' of ``atoms''. We observe that the common
denominator among all these data processing types (nested)
\textit{transformations} of (nested) \textit{collections}.  Moreover, even the
most optimized implementations can be described naturally in a nested way: inner
loops can be seen as the transformation of individual atoms of one collection
into another and the orchestration code around them as the nested compositions
of these transformations. Based on this observation, we built an abstraction for
multi-front-end multi-back-end data analysis.

We named this abstraction ``Collection Virtual Machine'' and we defined it as an
abstract virtual computer which uses registers to store ``collections'' and
executes linear sequences of ``instructions''.  These instructions can be seen
as transformations of the IR which must preserve its behavior \emph{as if it was
    executed on that machine}.

\begin{figure}[h]
    \centering
    \resizebox{0.4\textwidth}{!}{%
        \input{figures/cvm_arch}
    }%
    \caption{\textit{CVM} architecture}
    \label{fig:cvm_arch}
\end{figure}

Figure~\ref{fig:cvm_arch} depicts CVM high-level architecture. It has the
following main components:

\begin{description}

    \item[Front-ends] such that developers can use different dialects to specify
        their computations. Front-end examples can be a SQL interface, a DSL for
        doing graph processing, or any other DSL. Currently, we use a Python
        based DSL to express dataflow computations.

    \item[A collection-oriented intermediate representation (IR)] whose
        ``instructions'' are transformations of collections which we refer to as
        ``operators''.

    \item[An optimizer] which perform optimization passes over the IR while
        applying different optimization rules on each pass. During the final
        optimization pass, code is generated for the specific back-end.

    \item[Back-ends] can be (almost) anything to which our optimizer can lower
        the instructions to. Typical back-ends are x86, GPU or some other
        hardware specific back-end. Back-ends can also be software back-ends
        such as a database (our IR could be mapped into relational algebra
        expressions) or some other execution engine.

\end{description}

\subsection{Collection-oriented IR}
\label{subsec:cvm_ir}

Our virtual machine uses a set of instructions which perform
transformations over (nested) collections. Collections are of a generic type
with the following recursive structure:
%
\begin{equation}
  \varname{item} := \left\{\,
        \varname{atom} \,\middle|\,
        \varname{tuple}~\text{of}~\varname{items} \,\middle|\,
        \varname{collection}~\text{of}~\varname{items}
    \,\right\},
\end{equation}
%
where an \emph{atom} is an undividable value of a particular domain, a
\emph{tuple} is a mapping from a domain of names to items, and a
\emph{collection} is the generalization of any (abstract or concrete) data type
holding a finite, homogeneous multi-set. Where tuples types and collections
types can be denoted as follows:

\begin{table}[h]
    \begin{tabular}{ll}
        Tuple type:      &  $\langle\varname{fieldName0}: \varname{ItemType0},\,\ldots,\, $ \\
                         &  $\varname{fieldNameK}: \varname{ItemTypeK}\rangle$ \\
        Collection type: &  $\varname{CollectionType}\langle\varname{ItemType}\rangle$
    \end{tabular}
\end{table}

We define our virtual machine to have unlimited number of immutable registers.
Instructions use zero or many previously assigned registers to read collections
from and they can assign results to zero or many unassigned registers.
Moreover, these instructions may be parameterized with (constant) items or
programs. Thus, any instruction is of the following form:

\begin{algorithmic}
  \State $\varname{Out}_1$, \ldots, $\varname{Out}_m$
    $\gets$ \Call{Instruction}{$\varname{p}_1$, \ldots, $\varname{p}_k$}($\varname{In}_1$, \ldots, $\varname{In}_n$)
\end{algorithmic}

Here, $\varname{In}_i$ and $\varname{Out}_j$ are the input and output registers,
respectively, and all $\varname{p}_k$ are parameters. \footnote{For brevity, we
    omit empty components.}

In this way, programs can always be written in static single assignment (SSA)
form and if needed, a number of registers can be initialized with collections as
input parameters. Finally, its results can be returned using a special
instruction, \textsc{Return}($R_1$, \ldots, $R_n$).

\subsubsection{Collection types and instructions}

An important design decision we took regarding our collection-oriented IR is
that we deliberately let abstract and physical types and operators to co-exists
within the same IR.  This enables users to take advantage of their knowledge of
the data to choose the right (concrete) operator if possible.

\textbf{Abstract collection types} are used to express abstract data types such
as the ones in the upper part of table~\ref{tab:abs_cols}. For this, we define
the generic collection types \textit{Set, Bag, Seq} (for sequences), and
\textit{kDSeq} (for k-dimensional sequences) and use them to compose high-level
data types of various domains. 

\begin{table}[h]
  \centering
  \begin{tabular}{@{}l@{\hspace{1em}}l@{\hspace{1em}}l@{\hspace{-.5em}}}
    \toprule
    \textbf{Domain} & \textbf{Data structure} & \textbf{CVM data type} \\
    \midrule
    RA          & $R_1(A_1: D_1,\,\text{\ldots}\,A_k: D_k)$
                      & $\varname{Set}\langle A_1: D_1,\,\text{\ldots}\,A_k: D_k\rangle$ \\
    Bag RA      & $R_1(A_1: D_1,\,\text{\ldots}\,A_k: D_k)$
                      & $\varname{Bag}\langle A_1: D_1,\,\text{\ldots}\,A_k: D_k\rangle$ \\
    Seq. RA     & $R_1(A_1: D_1,\,\text{\ldots}\,A_k: D_k)$
                      & $\varname{Seq}\langle A_1: D_1,\,\text{\ldots}\,A_k: D_k\rangle$ \\
    \midrule
    RA (NF$^\text{2}$)
                      & $R_1(A: R_2(\text{\ldots}))$
                      & $\varname{Bag}\langle A_1: \varname{Bag}\langle\text{\ldots}\rangle\rangle$ \\
                      & $R(A_1: (A_2 : D))$
                      & $\varname{Bag}\langle A_1: \langle A_2 : D\rangle\rangle$ \\
%    LA          & $v \in \mathbb{R}$
%                      & $\varname{Seq}\langle\varname{Num}\rangle$ \\
%                      & $M \in \mathbb{R}^2$
%                      & $\varname{2DSeq}\langle\varname{Num}\rangle$ or \\
%                    & & $\varname{Seq}\langle\varname{Seq}\langle\varname{Num}\rangle\rangle$ \\
%                      & $M \in \mathbb{R}^k$
%                      & $\varname{kDSeq}\langle\varname{Num}\rangle$ or \\
%                    & & $\varname{Seq}\langle\text{\ldots}\,\varname{Seq}\langle\varname{Num}\rangle\text{\ldots}\rangle$ \\
    Graph             & $G = (V,E)$
                      & $\varname{Set}\langle\varname{ID}\rangle$ and \\
                    & & $\varname{Set}\langle\langle src: \varname{ID},\, dst: \varname{ID}\rangle\rangle$ \\
    \bottomrule\addlinespace[.5ex]

    \multicolumn{3}{c}{\small
        $R_i$: relation; $A_i$: attribute/field name; $D_i$: atomic domain
        } \\
  \end{tabular}
  \smallskip
  \caption{Abstract collection types.}
  \label{tab:abs_cols}
\end{table}

For example, relations from the original set-based relational algebra (RA) can
be expressed as \textit{Sets of tuples of atoms} where field names and types
represent the schema of the relation. Other more practical domains such as the
bag-based relational algebra or the non-first normal-form domain (NF$^2$ which
uses nested relations) can be expressed  using \textit{Bag} or \textit{Seq}
instead of sets and allowing nested non-atomic fields respectively.  Similarly,
we define vertices and edges of graphs where the collections' atoms have no
further structure, i.e., they are some type of vertex identifier
(\textit{ID}).

%vectors, matrices, and higher-dimensional tensors for linear algebra (LA), as
%well as the collections' atoms have no further structure, i.e., they are just
%some type of number (\textit{Num}) or vertex identifier (\textit{ID}).

\textbf{Physical collection types} are needed to express physical data layouts.
For representing an array of items in a single contiguous block of memory, we
define the generic type \emph{Vec}. Moreover, we express fixed-width records
with ordered fields (similar to \texttt{struct}s in C) as tuples where the
lexicographical order of the field names defines the physical order in the
layout.

For instance, row-store and column-store relation layouts are typically
implemented as \emph{array of structs} and \emph{struct of arrays} respectively,
which we can express with tuples and \emph{Vec}s.  We also define the generic
type \emph{Single} as a singleton collection holding just one tuple. This is
used as a helper to store a group of collections in a single register.

\begin{table}
  \centering
  \begin{tabular}{@{}l@{\hspace{1em}}l@{\hspace{1em}}l@{\hspace{-.5em}}}
    \toprule
    \textbf{Domain} & \textbf{Data structure} & \textbf{CVM data type} \\
    \midrule
    row-store   & \texttt{struct\{ D1 field1; \ldots \}}
                & $\langle v1 : D_1,\,v2 : \text{\ldots}\rangle$ \\
                & \texttt{struct\{ D1 field1; \ldots \}*}
                & $\varname{Vec}\langle\langle v1 : D_1,\,v2 : \text{\ldots}\rangle\rangle$ \\
    col-store   & \texttt{struct\{ D1* col1; \ldots \}}
                & $\varname{Single}\langle\langle v1 : \varname{Vec}\langle\varname{D_1}\rangle,\,\text{\ldots}\rangle\rangle$ \\
    %dense LA    & \texttt{float* A}
    %            & $\varname{Vec}\langle\varname{float}\rangle$ \\
    %            & \texttt{struct\{ int size[2];}
    %            & $\varname{Single}\langle\langle\varname{d1} : \varname{int},\,\varname{d2} : \varname{int},$ \\
    %            & \hspace{34pt}\texttt{float* A; \}}
    %            & \hspace{29pt}$A : \varname{Vec}\langle\varname{float}\rangle\rangle\rangle$ \\
    %sparse LA   & \texttt{struct\{ int nnz;}
    %            & $\varname{Single}\langle\langle A : \varname{Vec}\langle\varname{float}\rangle,$ \\
    %            & \hspace{12pt}\texttt{float* A; int* I;}
    %            & \hspace{32.5pt}$\varname{I} : \varname{Vec}\langle\varname{int}\rangle,$ \\
    %            & \hspace{12pt}\texttt{int* O; \}}
    %            & \hspace{29pt}$\varname{O} : \varname{Vec}\langle\varname{int}\rangle\rangle\rangle$ \\
    %SIMD        & \texttt{\_\_m256 v}
    %            & $\varname{Array8}\langle\varname{float}\rangle$ \\
    \bottomrule\addlinespace[.5ex]
    \multicolumn{3}{c}{\small
        $R$, $R_i$: relation; $A_i$, $A$: attribute/field name; $D_i$: atomic domain
        } \\
  \end{tabular}
  \smallskip
  \caption{Physical collection types.}
  \label{tbl:phy-collection-types}
\end{table}

The actual physical representation is decided by the backend. For this to
happen, the IR has to be brought into a form that the backend expects through
one of the active rewriting passes done over it. For example, a backend that
stores tuples of fixed-width fields using the memory layout of C-arrays of
C-structs would need the final IR to contain only \emph{Sequences} of anonymous
tuples to then lower these tuples accordingly.

\textbf{Custom collection types}

\subsubsection{Lowerings and rewritings}

\subsection{Extensions to IR}
\label{subsec:ir_extensions}
The operators that we need for running things in this setting.

\subsection{Optimization rules for serverless deployment}
\label{subsec:ir_opt_rules}
The optimization rules that make sense on this setting.

\begin{description}

    \item[Parallelization] moving operators into parallel scopes.
        \begin{figure}[h]
            \centering
            \resizebox{0.4\textwidth}{!}{%
                \input{figures/parallelize_rule}
            }%
        \end{figure}

    \item[Parallelization for AWS Lambda] moving input from cold storage.
        \begin{figure}[h]
            \centering
            \resizebox{0.5\textwidth}{!}{%
                \input{figures/parallel_aws_lambda}
            }%
        \end{figure}


\end{description}


==> figures/cvm_arch.tex <==



\tikzset{every picture/.style={line width=0.75pt}} %set default line width to 0.75pt        

\begin{tikzpicture}[x=0.75pt,y=0.75pt,yscale=-1,xscale=1]
%uncomment if require: \path (0,373); %set diagram left start at 0, and has height of 373

%Rounded Rect [id:dp6627378863922473] 
\draw   (35,19.6) .. controls (35,16.51) and (37.51,14) .. (40.6,14) -- (83.4,14) .. controls (86.49,14) and (89,16.51) .. (89,19.6) -- (89,36.4) .. controls (89,39.49) and (86.49,42) .. (83.4,42) -- (40.6,42) .. controls (37.51,42) and (35,39.49) .. (35,36.4) -- cycle ;

%Rounded Rect [id:dp08069135744999234] 
\draw   (173,19.6) .. controls (173,16.51) and (175.51,14) .. (178.6,14) -- (245.4,14) .. controls (248.49,14) and (251,16.51) .. (251,19.6) -- (251,36.4) .. controls (251,39.49) and (248.49,42) .. (245.4,42) -- (178.6,42) .. controls (175.51,42) and (173,39.49) .. (173,36.4) -- cycle ;

%Rounded Rect [id:dp24864756225891638] 
\draw   (255,19.6) .. controls (255,16.51) and (257.51,14) .. (260.6,14) -- (327.4,14) .. controls (330.49,14) and (333,16.51) .. (333,19.6) -- (333,36.4) .. controls (333,39.49) and (330.49,42) .. (327.4,42) -- (260.6,42) .. controls (257.51,42) and (255,39.49) .. (255,36.4) -- cycle ;

%Rounded Rect [id:dp08542150346061339] 
\draw   (337,19.6) .. controls (337,16.51) and (339.51,14) .. (342.6,14) -- (392.4,14) .. controls (395.49,14) and (398,16.51) .. (398,19.6) -- (398,36.4) .. controls (398,39.49) and (395.49,42) .. (392.4,42) -- (342.6,42) .. controls (339.51,42) and (337,39.49) .. (337,36.4) -- cycle ;

%Rounded Rect [id:dp962880961275987] 
\draw   (92,19.6) .. controls (92,16.51) and (94.51,14) .. (97.6,14) -- (164.4,14) .. controls (167.49,14) and (170,16.51) .. (170,19.6) -- (170,36.4) .. controls (170,39.49) and (167.49,42) .. (164.4,42) -- (97.6,42) .. controls (94.51,42) and (92,39.49) .. (92,36.4) -- cycle ;

%Rounded Rect [id:dp5129743434826273] 
\draw   (338,62.8) .. controls (338,60.7) and (339.7,59) .. (341.8,59) -- (395.2,59) .. controls (397.3,59) and (399,60.7) .. (399,62.8) -- (399,74.2) .. controls (399,76.3) and (397.3,78) .. (395.2,78) -- (341.8,78) .. controls (339.7,78) and (338,76.3) .. (338,74.2) -- cycle ;

%Straight Lines [id:da7185217395081032] 
\draw    (222,127) -- (222,143) ;
\draw [shift={(222,145)}, rotate = 270] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;

%Shape: Rectangle [id:dp4378552828397444] 
\draw   (40,95) -- (398,95) -- (398,126) -- (40,126) -- cycle ;

%Shape: Rectangle [id:dp08061082775879069] 
\draw   (41,209) -- (399,209) -- (399,249) -- (41,249) -- cycle ;

%Image [id:dp3449819855876666] 
\draw (221.63,167.05) node  {\includegraphics[width=19.3pt,height=14.81pt]{figures/gear-icon.png}};
%U Turn Arrow [id:dp36767419984886796] 
\draw   (199.83,168.95) -- (199.83,153.03) .. controls (199.83,149.26) and (202.89,146.2) .. (206.65,146.2) -- (237.9,146.2) .. controls (241.67,146.2) and (244.73,149.26) .. (244.73,153.03) -- (244.73,157.58) -- (247,157.58) -- (241.31,164.4) -- (235.63,157.58) -- (237.9,157.58) -- (237.9,153.03) .. controls (237.9,153.03) and (237.9,153.03) .. (237.9,153.03) -- (206.65,153.03) .. controls (206.65,153.03) and (206.65,153.03) .. (206.65,153.03) -- (206.65,168.95) -- cycle ;
%U Turn Arrow [id:dp08361623045588451] 
\draw   (244.17,167.64) -- (244.17,183.29) .. controls (244.17,187) and (241.17,190) .. (237.46,190) -- (205.94,190) .. controls (202.24,190) and (199.24,187) .. (199.24,183.29) -- (199.24,178.82) -- (197,178.82) -- (202.59,172.11) -- (208.18,178.82) -- (205.94,178.82) -- (205.94,183.29) .. controls (205.94,183.29) and (205.94,183.29) .. (205.94,183.29) -- (237.46,183.29) .. controls (237.46,183.29) and (237.46,183.29) .. (237.46,183.29) -- (237.46,167.64) -- cycle ;

%Straight Lines [id:da5695758208687214] 
\draw    (222,191) -- (222,207) ;
\draw [shift={(222,209)}, rotate = 270] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;

%Rounded Rect [id:dp6882513182698426] 
\draw   (61,270.8) .. controls (61,268.15) and (63.15,266) .. (65.8,266) -- (112.2,266) .. controls (114.85,266) and (117,268.15) .. (117,270.8) -- (117,285.2) .. controls (117,287.85) and (114.85,290) .. (112.2,290) -- (65.8,290) .. controls (63.15,290) and (61,287.85) .. (61,285.2) -- cycle ;

%Rounded Rect [id:dp6634365072299195] 
\draw   (133,270.8) .. controls (133,268.15) and (135.15,266) .. (137.8,266) -- (215.2,266) .. controls (217.85,266) and (220,268.15) .. (220,270.8) -- (220,285.2) .. controls (220,287.85) and (217.85,290) .. (215.2,290) -- (137.8,290) .. controls (135.15,290) and (133,287.85) .. (133,285.2) -- cycle ;

%Rounded Rect [id:dp027299728427228498] 
\draw   (235,270.8) .. controls (235,268.15) and (237.15,266) .. (239.8,266) -- (379.2,266) .. controls (381.85,266) and (384,268.15) .. (384,270.8) -- (384,285.2) .. controls (384,287.85) and (381.85,290) .. (379.2,290) -- (239.8,290) .. controls (237.15,290) and (235,287.85) .. (235,285.2) -- cycle ;

%Rounded Rect [id:dp6288920035820131] 
\draw   (66,309.8) .. controls (66,307.15) and (68.15,305) .. (70.8,305) -- (153.2,305) .. controls (155.85,305) and (158,307.15) .. (158,309.8) -- (158,324.2) .. controls (158,326.85) and (155.85,329) .. (153.2,329) -- (70.8,329) .. controls (68.15,329) and (66,326.85) .. (66,324.2) -- cycle ;

%Rounded Rect [id:dp3196731960939383] 
\draw   (170,309.8) .. controls (170,307.15) and (172.15,305) .. (174.8,305) -- (257.2,305) .. controls (259.85,305) and (262,307.15) .. (262,309.8) -- (262,324.2) .. controls (262,326.85) and (259.85,329) .. (257.2,329) -- (174.8,329) .. controls (172.15,329) and (170,326.85) .. (170,324.2) -- cycle ;

%Rounded Rect [id:dp06486110867239758] 
\draw   (274,309.8) .. controls (274,307.15) and (276.15,305) .. (278.8,305) -- (361.2,305) .. controls (363.85,305) and (366,307.15) .. (366,309.8) -- (366,324.2) .. controls (366,326.85) and (363.85,329) .. (361.2,329) -- (278.8,329) .. controls (276.15,329) and (274,326.85) .. (274,324.2) -- cycle ;

%Straight Lines [id:da6754571671975009] 
\draw    (62,43) -- (62,92) ;
\draw [shift={(62,94)}, rotate = 270] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;

%Straight Lines [id:da31373823700619674] 
\draw    (131,43) -- (131,93) ;
\draw [shift={(131,95)}, rotate = 270] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;

%Straight Lines [id:da7897439885198476] 
\draw    (210,43) -- (210,92) ;
\draw [shift={(210,94)}, rotate = 270] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;

%Straight Lines [id:da9018791390319787] 
\draw    (294,43) -- (294,92) ;
\draw [shift={(294,94)}, rotate = 270] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;

%Straight Lines [id:da6523806503467293] 
\draw    (367,42) -- (367,57) ;
\draw [shift={(367,59)}, rotate = 270] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;

%Straight Lines [id:da8508341082470476] 
\draw    (367,78) -- (367,93) ;
\draw [shift={(367,95)}, rotate = 270] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;

%Curve Lines [id:da10744480285838498] 
\draw    (201,250) .. controls (179.55,253.9) and (118.17,254.95) .. (93.8,264.27) ;
\draw [shift={(92,265)}, rotate = 336.5] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;

%Curve Lines [id:da7674039853985253] 
\draw    (225,250) .. controls (221.22,246.22) and (196.9,253.16) .. (194.24,264.06) ;
\draw [shift={(194,266)}, rotate = 270] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;

%Curve Lines [id:da3626561256287686] 
\draw    (242,249) .. controls (248.86,261.74) and (275.89,254.31) .. (305.2,264.36) ;
\draw [shift={(307,265)}, rotate = 200.14] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;


% Text Node
\draw (62,28) node  [align=left] {SQL};
% Text Node
\draw (210.95,28) node  [align=left] {LinearAlg.};
% Text Node
\draw (292.95,28) node  [align=left] {Dataflow};
% Text Node
\draw (366.68,28) node  [align=left] {Graph};
% Text Node
\draw (129.95,28) node  [align=left] {JSONiq};
% Text Node
\draw (367.68,68.5) node  [align=left] {lib};
% Text Node
\draw (219,110.5) node  [align=left] {Input program (Intermediate Representation)};
% Text Node
\draw (220,229) node  [align=left] {Output program (Intermediate Representation)};
% Text Node
\draw (279,165) node  [align=left] {\textit{optimization}\\\textit{passes}};
% Text Node
\draw (91,278) node  [align=left] {{\small VMs}};
% Text Node
\draw (176,278) node  [align=left] {{\small Containers}};
% Text Node
\draw (308.64,278) node  [align=left] {{\small Serverless Functions}};
% Text Node
\draw (111.68,317) node  [align=left] {{\small LocalStorage}};
% Text Node
\draw (215.68,317) node  [align=left] {{\small ObjectStore}};
% Text Node
\draw (319.68,317) node  [align=left] {{\small QueueService}};
% Text Node
\draw (92,296) node  [align=left] {$\displaystyle \times $};
% Text Node
\draw (181,296) node  [align=left] {$\displaystyle \times $};
% Text Node
\draw (305,296) node  [align=left] {$\displaystyle \times $};


\end{tikzpicture}



==> figures/parallel_aws_lambda.tex <==
\tikzset{every picture/.style={line width=0.75pt}} %set default line width to 0.75pt        

\begin{tikzpicture}[x=0.75pt,y=0.75pt,yscale=-1,xscale=1]
%uncomment if require: \path (0,508); %set diagram left start at 0, and has height of 508

%Shape: Ellipse [id:dp8904923695165996] 
\draw   (81,56.5) .. controls (81,45.18) and (107.86,36) .. (141,36) .. controls (174.14,36) and (201,45.18) .. (201,56.5) .. controls (201,67.82) and (174.14,77) .. (141,77) .. controls (107.86,77) and (81,67.82) .. (81,56.5) -- cycle ;

%Shape: Ellipse [id:dp2345984805298833] 
\draw   (268,86.5) .. controls (268,76.28) and (300.46,68) .. (340.5,68) .. controls (380.54,68) and (413,76.28) .. (413,86.5) .. controls (413,96.72) and (380.54,105) .. (340.5,105) .. controls (300.46,105) and (268,96.72) .. (268,86.5) -- cycle ;

%Shape: Ellipse [id:dp07041547354171374] 
\draw   (80,287) .. controls (80,278.16) and (106.86,271) .. (140,271) .. controls (173.14,271) and (200,278.16) .. (200,287) .. controls (200,295.84) and (173.14,303) .. (140,303) .. controls (106.86,303) and (80,295.84) .. (80,287) -- cycle ;

%Straight Lines [id:da5915722518571622] 
\draw    (141,77) -- (140.1,95) ;
\draw [shift={(140,97)}, rotate = 272.86] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;

%Shape: Ellipse [id:dp8885257199996792] 
\draw  [color={rgb, 255:red, 5; green, 77; blue, 168 }  ,draw opacity=1 ][line width=1.5]  (41,119) .. controls (41,106.85) and (85.32,97) .. (140,97) .. controls (194.68,97) and (239,106.85) .. (239,119) .. controls (239,131.15) and (194.68,141) .. (140,141) .. controls (85.32,141) and (41,131.15) .. (41,119) -- cycle ;

%Shape: Ellipse [id:dp414363628202588] 
\draw   (298,33.5) .. controls (298,23.28) and (316.8,15) .. (340,15) .. controls (363.2,15) and (382,23.28) .. (382,33.5) .. controls (382,43.72) and (363.2,52) .. (340,52) .. controls (316.8,52) and (298,43.72) .. (298,33.5) -- cycle ;

%Straight Lines [id:da059142175258574126] 
\draw    (342,210.5) -- (342,222) ;
\draw [shift={(342,224)}, rotate = 270] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;

%Shape: Ellipse [id:dp08548350040701891] 
\draw   (300,242.5) .. controls (300,232.28) and (318.8,224) .. (342,224) .. controls (365.2,224) and (384,232.28) .. (384,242.5) .. controls (384,252.72) and (365.2,261) .. (342,261) .. controls (318.8,261) and (300,252.72) .. (300,242.5) -- cycle ;


%Shape: Ellipse [id:dp09291236986136209] 
\draw  [color={rgb, 255:red, 65; green, 117; blue, 5 }  ,draw opacity=1 ][line width=1.5]  (266,138) .. controls (266,127.78) and (299.58,119.5) .. (341,119.5) .. controls (382.42,119.5) and (416,127.78) .. (416,138) .. controls (416,148.22) and (382.42,156.5) .. (341,156.5) .. controls (299.58,156.5) and (266,148.22) .. (266,138) -- cycle ;

%Straight Lines [id:da8441184465532536] 
\draw    (139,251) -- (139.9,269) ;
\draw [shift={(140,271)}, rotate = 267.14] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;

%Shape: Ellipse [id:dp27798199197750373] 
\draw   (79,230.5) .. controls (79,219.73) and (105.86,211) .. (139,211) .. controls (172.14,211) and (199,219.73) .. (199,230.5) .. controls (199,241.27) and (172.14,250) .. (139,250) .. controls (105.86,250) and (79,241.27) .. (79,230.5) -- cycle ;

%Straight Lines [id:da3161408632707059] 
\draw    (138,191) -- (138,209) ;
\draw [shift={(138,211)}, rotate = 270] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;

%Shape: Ellipse [id:dp6206452333303356] 
\draw   (79,174.62) .. controls (79,165.58) and (105.86,158.25) .. (139,158.25) .. controls (172.14,158.25) and (199,165.58) .. (199,174.62) .. controls (199,183.67) and (172.14,191) .. (139,191) .. controls (105.86,191) and (79,183.67) .. (79,174.62) -- cycle ;

%Straight Lines [id:da9179737895162672] 
\draw    (140,140) -- (139.11,156.25) ;
\draw [shift={(139,158.25)}, rotate = 273.14] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;

%Shape: Ellipse [id:dp8944117912802674] 
\draw  [color={rgb, 255:red, 65; green, 117; blue, 5 }  ,draw opacity=1 ][line width=1.5]  (267,192) .. controls (267,181.78) and (300.58,173.5) .. (342,173.5) .. controls (383.42,173.5) and (417,181.78) .. (417,192) .. controls (417,202.22) and (383.42,210.5) .. (342,210.5) .. controls (300.58,210.5) and (267,202.22) .. (267,192) -- cycle ;

%Straight Lines [id:da4948940157282775] 
\draw    (341,156.5) -- (341.88,171.5) ;
\draw [shift={(342,173.5)}, rotate = 266.63] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;

%Straight Lines [id:da48611574698269155] 
\draw    (340.5,105) -- (339.17,120.51) ;
\draw [shift={(339,122.5)}, rotate = 274.9] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;

%Straight Lines [id:da9068616843077273] 
\draw    (340,52) -- (340.44,66) ;
\draw [shift={(340.5,68)}, rotate = 268.21] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;

%Straight Lines [id:da01211206943934462] 
\draw    (342.68,261.5) -- (342.68,273) ;
\draw [shift={(342.68,275)}, rotate = 270] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;

%Shape: Ellipse [id:dp7800964590702051] 
\draw   (274.12,293.5) .. controls (274.12,283.28) and (304.82,275) .. (342.68,275) .. controls (380.55,275) and (411.25,283.28) .. (411.25,293.5) .. controls (411.25,303.72) and (380.55,312) .. (342.68,312) .. controls (304.82,312) and (274.12,303.72) .. (274.12,293.5) -- cycle ;


%Shape: Ellipse [id:dp9548516723421234] 
\draw   (476,86.5) .. controls (476,76.28) and (508.46,68) .. (548.5,68) .. controls (588.54,68) and (621,76.28) .. (621,86.5) .. controls (621,96.72) and (588.54,105) .. (548.5,105) .. controls (508.46,105) and (476,96.72) .. (476,86.5) -- cycle ;

%Shape: Ellipse [id:dp9277265914375386] 
\draw   (506,33.5) .. controls (506,23.28) and (524.8,15) .. (548,15) .. controls (571.2,15) and (590,23.28) .. (590,33.5) .. controls (590,43.72) and (571.2,52) .. (548,52) .. controls (524.8,52) and (506,43.72) .. (506,33.5) -- cycle ;

%Straight Lines [id:da34528389666204284] 
\draw    (550,210.5) -- (550,222) ;
\draw [shift={(550,224)}, rotate = 270] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;

%Shape: Ellipse [id:dp125968045036976] 
\draw   (508,242.5) .. controls (508,232.28) and (526.8,224) .. (550,224) .. controls (573.2,224) and (592,232.28) .. (592,242.5) .. controls (592,252.72) and (573.2,261) .. (550,261) .. controls (526.8,261) and (508,252.72) .. (508,242.5) -- cycle ;


%Shape: Ellipse [id:dp6388534707294982] 
\draw  [color={rgb, 255:red, 32; green, 39; blue, 155 }  ,draw opacity=1 ][line width=1.5]  (474,138) .. controls (474,127.78) and (507.58,119.5) .. (549,119.5) .. controls (590.42,119.5) and (624,127.78) .. (624,138) .. controls (624,148.22) and (590.42,156.5) .. (549,156.5) .. controls (507.58,156.5) and (474,148.22) .. (474,138) -- cycle ;

%Shape: Ellipse [id:dp28612469130425633] 
\draw  [color={rgb, 255:red, 12; green, 25; blue, 158 }  ,draw opacity=1 ][line width=1.5]  (475,192) .. controls (475,181.78) and (508.58,173.5) .. (550,173.5) .. controls (591.42,173.5) and (625,181.78) .. (625,192) .. controls (625,202.22) and (591.42,210.5) .. (550,210.5) .. controls (508.58,210.5) and (475,202.22) .. (475,192) -- cycle ;

%Straight Lines [id:da967196848778064] 
\draw    (548,156.5) -- (548.88,171.5) ;
\draw [shift={(549,173.5)}, rotate = 266.63] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;

%Straight Lines [id:da19598952038827222] 
\draw    (548.5,105) -- (548.07,117.5) ;
\draw [shift={(548,119.5)}, rotate = 271.97] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;

%Straight Lines [id:da19761657301743996] 
\draw    (547,52) -- (547.44,66) ;
\draw [shift={(547.5,68)}, rotate = 268.21] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;

%Straight Lines [id:da450324398790213] 
\draw    (550.06,261.5) -- (550.06,273) ;
\draw [shift={(550.06,275)}, rotate = 270] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;

%Shape: Ellipse [id:dp3842391669297789] 
\draw   (470.12,293.5) .. controls (470.12,283.28) and (505.91,275) .. (550.06,275) .. controls (594.21,275) and (630,283.28) .. (630,293.5) .. controls (630,303.72) and (594.21,312) .. (550.06,312) .. controls (505.91,312) and (470.12,303.72) .. (470.12,293.5) -- cycle ;


%Right Arrow [id:dp4311424924196787] 
\draw  [color={rgb, 255:red, 0; green, 0; blue, 0 }  ,draw opacity=1 ][line width=1.5]  (421,156.25) -- (454,156.25) -- (454,150) -- (468,162.5) -- (454,175) -- (454,168.75) -- (421,168.75) -- cycle ;
%Shape: Brace [id:dp1757156676356686] 
\draw  [color={rgb, 255:red, 0; green, 0; blue, 0 }  ,draw opacity=1 ][line width=1.5]  (259,17) .. controls (254.33,17.03) and (252.02,19.38) .. (252.05,24.05) -- (252.6,107.96) .. controls (252.65,114.63) and (250.34,117.97) .. (245.67,118) .. controls (250.34,117.97) and (252.69,121.29) .. (252.74,127.96)(252.72,124.96) -- (253.96,312.05) .. controls (253.99,316.72) and (256.33,319.03) .. (261,319) ;

% Text Node
\draw (142,56.5) node  [align=left] {Param\_Lookup};
% Text Node
\draw (339.5,33) node  [align=left] {Map};
% Text Node
\draw (339.5,87) node  [align=left] {Local\_Partitioning};
% Text Node
\draw (140,287) node  [align=left] {Materialize};
% Text Node
\draw (140,119.81) node  [align=left] {\textcolor[rgb]{0.03,0.13,0.63}{\textit{Parallel\_Aws\_LambdaMap}}};
% Text Node
\draw (341,138) node  [align=left] {\textcolor[rgb]{0.25,0.46,0.02}{Materialize\_S3}};
% Text Node
\draw (139,230.5) node  [align=left] {Read\_S3\_File};
% Text Node
\draw (142,172.62) node  [align=left] {Row\_scan};
% Text Node
\draw (342.5,243) node  [align=left] {Reduce};
% Text Node
\draw (342,192) node  [align=left] {\textcolor[rgb]{0.25,0.46,0.02}{Read\_S3}};
% Text Node
\draw (343.5,294) node  [align=left] {Materialize\_S3};
% Text Node
\draw (551.01,294) node  [align=left] {Materialize\_S3\_File};
% Text Node
\draw (550,192) node  [align=left] {\textcolor[rgb]{0.05,0.13,0.62}{Read\_S3\_File}};
% Text Node
\draw (549,138) node  [align=left] {\textcolor[rgb]{0.05,0.13,0.62}{Materialize\_S3\_File}};
% Text Node
\draw (550.5,243) node  [align=left] {Reduce};
% Text Node
\draw (547.5,33) node  [align=left] {Map};
% Text Node
\draw (547.5,87) node  [align=left] {Local\_Partitioning};


\end{tikzpicture}



==> figures/parallelize_rule.tex <==


\tikzset{every picture/.style={line width=0.75pt}} %set default line width to 0.75pt        

\begin{tikzpicture}[x=0.75pt,y=0.75pt,yscale=-1,xscale=1]
%uncomment if require: \path (0,431); %set diagram left start at 0, and has height of 431

%Shape: Ellipse [id:dp3409026869852121] 
\draw   (52,63) .. controls (52,45.88) and (78.86,32) .. (112,32) .. controls (145.14,32) and (172,45.88) .. (172,63) .. controls (172,80.12) and (145.14,94) .. (112,94) .. controls (78.86,94) and (52,80.12) .. (52,63) -- cycle ;
%Shape: Ellipse [id:dp04655867306080341] 
\draw   (51,140) .. controls (51,122.88) and (77.86,109) .. (111,109) .. controls (144.14,109) and (171,122.88) .. (171,140) .. controls (171,157.12) and (144.14,171) .. (111,171) .. controls (77.86,171) and (51,157.12) .. (51,140) -- cycle ;
%Shape: Ellipse [id:dp05100981983146169] 
\draw   (51,215) .. controls (51,197.88) and (77.86,184) .. (111,184) .. controls (144.14,184) and (171,197.88) .. (171,215) .. controls (171,232.12) and (144.14,246) .. (111,246) .. controls (77.86,246) and (51,232.12) .. (51,215) -- cycle ;
%Shape: Ellipse [id:dp17646590122109962] 
\draw   (52,294) .. controls (52,276.88) and (78.86,263) .. (112,263) .. controls (145.14,263) and (172,276.88) .. (172,294) .. controls (172,311.12) and (145.14,325) .. (112,325) .. controls (78.86,325) and (52,311.12) .. (52,294) -- cycle ;
%Straight Lines [id:da3419815023943069] 
\draw    (112,94) -- (111.13,107) ;
\draw [shift={(111,109)}, rotate = 273.81] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;

%Straight Lines [id:da08460746809513031] 
\draw    (111,171) -- (111,182) ;
\draw [shift={(111,184)}, rotate = 270] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;

%Straight Lines [id:da8110381150119785] 
\draw    (111,246) -- (111.88,261) ;
\draw [shift={(112,263)}, rotate = 266.63] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;

%Shape: Ellipse [id:dp9244676244715897] 
\draw   (236,65) .. controls (236,47.88) and (262.86,34) .. (296,34) .. controls (329.14,34) and (356,47.88) .. (356,65) .. controls (356,82.12) and (329.14,96) .. (296,96) .. controls (262.86,96) and (236,82.12) .. (236,65) -- cycle ;
%Shape: Ellipse [id:dp03656272138446903] 
\draw   (254,233.5) .. controls (254,223.28) and (272.8,215) .. (296,215) .. controls (319.2,215) and (338,223.28) .. (338,233.5) .. controls (338,243.72) and (319.2,252) .. (296,252) .. controls (272.8,252) and (254,243.72) .. (254,233.5) -- cycle ;
%Shape: Ellipse [id:dp29118677205133303] 
\draw   (238,373) .. controls (238,355.88) and (264.86,342) .. (298,342) .. controls (331.14,342) and (358,355.88) .. (358,373) .. controls (358,390.12) and (331.14,404) .. (298,404) .. controls (264.86,404) and (238,390.12) .. (238,373) -- cycle ;
%Straight Lines [id:da705374952064246] 
\draw    (296,96) -- (296.9,114) ;
\draw [shift={(297,116)}, rotate = 267.14] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;

%Straight Lines [id:da8318438729829989] 
\draw    (298,197) -- (296.22,213.01) ;
\draw [shift={(296,215)}, rotate = 276.34000000000003] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;

%Shape: Ellipse [id:dp9111657781228548] 
\draw   (221,219.5) .. controls (221,162.34) and (255.03,116) .. (297,116) .. controls (338.97,116) and (373,162.34) .. (373,219.5) .. controls (373,276.66) and (338.97,323) .. (297,323) .. controls (255.03,323) and (221,276.66) .. (221,219.5) -- cycle ;
%Shape: Ellipse [id:dp41711727877871163] 
\draw   (256,180.5) .. controls (256,170.28) and (274.8,162) .. (298,162) .. controls (321.2,162) and (340,170.28) .. (340,180.5) .. controls (340,190.72) and (321.2,199) .. (298,199) .. controls (274.8,199) and (256,190.72) .. (256,180.5) -- cycle ;
%Straight Lines [id:da1801020715237287] 
\draw    (296,252) -- (296.89,267.5) ;
\draw [shift={(297,269.5)}, rotate = 266.73] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;

%Shape: Ellipse [id:dp8521990324271418] 
\draw   (255,288) .. controls (255,277.78) and (273.8,269.5) .. (297,269.5) .. controls (320.2,269.5) and (339,277.78) .. (339,288) .. controls (339,298.22) and (320.2,306.5) .. (297,306.5) .. controls (273.8,306.5) and (255,298.22) .. (255,288) -- cycle ;
%Straight Lines [id:da31138607650809447] 
\draw    (297,323) -- (297.9,341) ;
\draw [shift={(298,343)}, rotate = 267.14] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;

%Shape: Ellipse [id:dp10770053018817038] 
\draw   (436,65) .. controls (436,47.88) and (462.86,34) .. (496,34) .. controls (529.14,34) and (556,47.88) .. (556,65) .. controls (556,82.12) and (529.14,96) .. (496,96) .. controls (462.86,96) and (436,82.12) .. (436,65) -- cycle ;
%Shape: Ellipse [id:dp06905918458063032] 
\draw   (454,233.5) .. controls (454,223.28) and (472.8,215) .. (496,215) .. controls (519.2,215) and (538,223.28) .. (538,233.5) .. controls (538,243.72) and (519.2,252) .. (496,252) .. controls (472.8,252) and (454,243.72) .. (454,233.5) -- cycle ;
%Shape: Ellipse [id:dp1969455742884969] 
\draw   (438,373) .. controls (438,355.88) and (464.86,342) .. (498,342) .. controls (531.14,342) and (558,355.88) .. (558,373) .. controls (558,390.12) and (531.14,404) .. (498,404) .. controls (464.86,404) and (438,390.12) .. (438,373) -- cycle ;
%Straight Lines [id:da3013300219995301] 
\draw    (496,96) -- (496.9,114) ;
\draw [shift={(497,116)}, rotate = 267.14] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;

%Straight Lines [id:da27161159867064133] 
\draw    (498,197) -- (496.22,213.01) ;
\draw [shift={(496,215)}, rotate = 276.34000000000003] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;

%Shape: Ellipse [id:dp9917365262696549] 
\draw   (421,219.5) .. controls (421,162.34) and (455.7,116) .. (498.5,116) .. controls (541.3,116) and (576,162.34) .. (576,219.5) .. controls (576,276.66) and (541.3,323) .. (498.5,323) .. controls (455.7,323) and (421,276.66) .. (421,219.5) -- cycle ;
%Shape: Ellipse [id:dp9463441717269276] 
\draw   (456,180.5) .. controls (456,170.28) and (474.8,162) .. (498,162) .. controls (521.2,162) and (540,170.28) .. (540,180.5) .. controls (540,190.72) and (521.2,199) .. (498,199) .. controls (474.8,199) and (456,190.72) .. (456,180.5) -- cycle ;
%Straight Lines [id:da8465738106040506] 
\draw    (496,252) -- (496.89,267.5) ;
\draw [shift={(497,269.5)}, rotate = 266.73] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;

%Shape: Ellipse [id:dp8426815258635509] 
\draw   (455,288) .. controls (455,277.78) and (473.8,269.5) .. (497,269.5) .. controls (520.2,269.5) and (539,277.78) .. (539,288) .. controls (539,298.22) and (520.2,306.5) .. (497,306.5) .. controls (473.8,306.5) and (455,298.22) .. (455,288) -- cycle ;
%Straight Lines [id:da12307620817067111] 
\draw    (497,323) -- (497.9,341) ;
\draw [shift={(498,343)}, rotate = 267.14] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;

%Right Arrow [id:dp8212812951547157] 
\draw   (184,174.75) -- (202.6,174.75) -- (202.6,168) -- (215,181.5) -- (202.6,195) -- (202.6,188.25) -- (184,188.25) -- cycle ;
%Right Arrow [id:dp4219708740810362] 
\draw   (385,174.75) -- (403.6,174.75) -- (403.6,168) -- (416,181.5) -- (403.6,195) -- (403.6,188.25) -- (385,188.25) -- cycle ;

% Text Node
\draw (112.5,62) node  [align=left] {Param\_Lookup};
% Text Node
\draw (110.5,140) node  [align=left] {Map};
% Text Node
\draw (110.5,217) node  [align=left] {Reduce};
% Text Node
\draw (112.5,293) node  [align=left] {Materialize};
% Text Node
\draw (297,65) node  [align=left] {Param\_Lookup};
% Text Node
\draw (297.5,180) node  [align=left] {Map};
% Text Node
\draw (294.5,234) node  [align=left] {Reduce};
% Text Node
\draw (298,373) node  [align=left] {Materialize};
% Text Node
\draw (298,145) node  [align=left] {\textcolor[rgb]{0,0,0}{\textbf{Parallel\_Map}}};
% Text Node
\draw (297,289) node  [align=left] {Materialize};
% Text Node
\draw (497,65) node  [align=left] {Param\_Lookup};
% Text Node
\draw (497.5,180) node  [align=left] {Map};
% Text Node
\draw (494.5,234) node  [align=left] {Reduce};
% Text Node
\draw (498,373) node  [align=left] {Materialize};
% Text Node
\draw (498,145) node [color={rgb, 255:red, 0; green, 0; blue, 0 }  ,opacity=1 ] [align=left] {\textbf{Parallel\_AWS\_LambdaMap}};
% Text Node
\draw (497,289) node  [align=left] {Materialize};


\end{tikzpicture}


